On supercuspidal representations of $SL_n(F)$ associated with tamely ramified extensions

We will give an explicit construction of irreducible suparcuspidal representations of the special linear group over a non-archimedean local field and will speculate its Langlands parameter by means of verifying the Hiraga-Ichino-Ikeda formula of the formal degree of the supercuspidal representations.

==> front.tex <==
\section{Introduction}
\label{sec:introduction}

\subsection[]{}
Although the $L$-packets of the
irreducible supercuspidal representations of the special linear group
over non-archimedean local field  are well-understood
by the works of \cite{LabesseLanglands1979}, \cite{GelbartKnapp1982}, 
\cite{MoySally1984} or by \cite{HiragaSaito2012}, 
little is known for explicit determination of
the Langlands parameter of an individual explicitly constructed
supercuspidal representation. In this paper, we will construct quite
explicitely some supercuspidal representations, 
associated with tamely ramified extensions, 
of the special linear
group over non-archimedean local field and will speculate its 
Langlands parameter by showing the formula of the formal degree
established by Hiraga, Ichino and Ikeda \cite{HiragaSaito2012}. 

\subsection[]{}
The main results of this paper are Theorem 
\ref

